Unit Perturbations in Budgeted Spanning Tree Problems

The minimum spanning tree of a graph is a well-studied structure that is the basis of countless graph theoretic and optimization problem. We study the minimum spanning tree (MST) perturbation problem where the goal is to spend a fixed budget to increase the weight of edges in order to increase the weight of the MST as much as possible. Two popular models of perturbation are bulk and continuous. In the bulk model, the weight of any edge can be increased exactly once to some predetermined weight. In the continuous model, one can pay a fractional amount of cost to increase the weight of any edge by a proportional amount. Frederickson and Solis-Oba \cite{FS96} have studied these two models and showed that bulk perturbation for MST is as hard as the $k$-cut problem while the continuous perturbation model is solvable in poly-time. In this paper, we study an intermediate unit perturbation variation of this problem where the weight of each edge can be increased many times but at an integral unit amount every time. We provide an $(opt/2 -1)$-approximation in polynomial time where $opt$ is the optimal increase in the weight. We also study the associated dual targeted version of the problem where the goal is to increase the weight of the MST by a target amount while minimizing the cost of perturbation. We provide a $2$-approximation for this variation. Furthermore we show that assuming the Small Set Expansion Hypothesis, both problems are hard to approximate. We also point out an error in the proof provided by Frederickson and Solis-Oba in \cite{FS96} with regard to their solution to the continuous perturbation model. Although their algorithm is correct, their analysis is flawed. We provide a correct proof here.

==> MSAUpgrading.tex <==
\section{Related Problems}

\subsection{Downgrading MSA in Directed Graphs}

Consider the directed analogy of the MST Downgrading problem:

\begin{problem} (MMSA)
	Given a directed graph $G$, a root $r$, functions $w, c:A(G)\to \mathbb{N}$ and a budget $B$, find a downgrading scheme $x:A(G)\to \mathbb{N}$ that maximizes $f_x$, the weight of a minimum spanning $r$-arborescent in $(G,w+x)$ while ensuring the total cost $c_x := c \cdot x \le B$.

\end{problem}



\iffalse_______________________
\subsection{When $G$ is a DAG}
In this subsection, let us consider the special case of MMSA where the input graph $G$ is a directed acyclic graph.

\begin{theorem}
    If $G$ is a directed acycle graph, then MMSA can be solved in strongly polynomial time. 
\end{theorem}

\begin{proof}
Let $x^*$ be an optimal solution and $T^*$ be the increase in the value of the MSA due to $x^*$. Let us first analyze the structures of this solution. With the final weights of $w+x^*$, a MSA can be constructed by simply taking the least weighted ingoing arc adjacent to each vertex. It is easy to see that this constructs an $r$-arborescent since the graph is a DAG. One can also easily check that it provides a minimum spanning arborescnet. Then, if an arc $uv$ is downgraded, there is no need to increase its value beyond the minimum final weight of all ingoing arcs incident to $v$. In other words, for all ingoing arcs with non-zero $x^*$ value incident to $v$, their final weights are the same and is the minimum of all ingoing arcs to $v$ with respect to the final weight. Let $m_v$ be the value of the smallest weight of ingoing arcs to $v$ with respect to the initial weight $w$. Let $M_v$ be the value of the smallest weight of ingoing arcs to $v$ with respect to the final weight $w+x^*$. Note that the initial MSA value is $\sum_v m_v$ while the final MSA value is $\sum_v M_v$. Thus, $T^*=\sum_v(M_v-m_v)$. Then, our algorithm will attempt to find the best way to reach $T^*$ by determining the corresponding $M_v$ values.

Slightly abusing the notation, let $x_v$ denote the targeted change in the minimum weight of all ingoing arcs of $v$. Our goal is to find the cheapest way to assign $x_v$ such that $\sum_v x_v$ reaches our target increase in total MSA value. Note that in order to achieve a certain value of $x_v$, one must increase all arcs of weight strictly less than $m_v+x_v$ to the value $x_v$. Then, the incremental cost of changing $x_v$ to $x_v+1$ is $\sum_{uv: w(uv)\le m_v+x_v} c(uv)$, where we bump up the value of all edges whose starting weight is strictly less than $x_v-1$ one more time. Then, we can use dynamic programming to solve this problem. 

Let $T$ denote the targeted total increase in the value of the MSA. We first use dynamic programming to find all possible combinations for achieving $T$ when $T\le n^3$. 


\end{proof}
_______________________________________
\fi

\subsection{$k$-Blocker for MST and $k+1$-Cut

Consider the $k$-blocker for MST:

\begin{definition}
    A set of edges $F$ is a $k$-blocker for MST of a graph $G$ if $F\cap T\ge k$ for every MST $T$. 
\end{definition}

\begin{problem} (MSTkB)
    Given a graph $G$ with edge weights $w$ and edge costs $c$, find a $k$-blocker of MST (with respect to $w$) of $G$ with minimum cost with respect to $c$. 
\end{problem}

\begin{proposition}
    MSTkB is as hard as $k+1$-cut. 
\end{proposition}

\begin{proof}
    For $i\in \mathbb{N}$, let $G_i$ be the graph obtained by contracting every edge of weight strictly less than $i$ and deleting all edges with weight strictly larger than $i$. Create $G'$ by adding a dummy node $s$ and for every $i$, and every connected component in $G_i$, pick an arbitrary vertex and connect it to $s$ with an edge with infinite cost. Now we show that a minimum cost $k+1$-cut in $G'$ corresponds to a minimum cost $k$-blocker for $$MST in $G$.
    
    First we will show that a $k$-blocker is a $k+1$ cut. Let $F$ be a $k$-blocker. Let $H$ be a connected component of $G_i$. Note that for any MST $T$, $T$ restricted to $H$ is also a spanning tree. Let $k_H$ be the minimum number of times $F\cap H$ blocks the spanning trees of $H$. Note that $\sum_H k_H=k$. 
\end{proof}

==> MSTUpgrading.tex <==
\section{Downgrading MSTs in undirected graphs}



% TODO: DaQi adds new section on directed spanning trees

==> MinCutUpgrading.tex <==
\section{Upgrading Cuts and Paths}
\subsection{Upgrading $st$-Minimum Cuts}

\begin{problem} (MaxMC)
	Given a graph $G$ and $s, t\in V$, let $w, c :E\to \mathbb{N}$ respectively represent the original capacity and the cost of unit upgrading. Given a budget $B\in\mathbb{N}$, find an edge set $X$ to upgrade such that $\sum_{e \in X} c(x)\le B$ and the minimum $st$-cut after upgrading the capacities in $X$ is maximum.
\end{problem}

We can see this as $f = \text{MinCut weight}$, and $u \equiv 1$. For any upgraded edge $e$, the weight will be $w(e)+1$



%\subsection{Smooth MinCut Upgrade is poly time for unitary upgrade amounts}

%\begin{lemma}
%	Upper bounded Smooth MaxMC is polytime solvable.
%\end{lemma}

%\begin{proof}
%	We reduce the problem to Minimum Cost Flows. First, we guess the value of the optimal final min-cut (max-flow) $f^*$ on spending the budget. Construct $G'$ by adding a parallel edge $e'$ to every edge $e$. Every original edge has capacity $c(e)$ and cost $0$ and every new edge has cost $r(e)$ and capacity $1$. Then, compute the minimum cost to achieve a flow of $f^*$. Note that this solution is integral. If the cost is more than $b$ we know $f^*$ is not attainable. Then, using binary search, one can find the maximum $f^*$ that is attainable with budget $B$ and thus also find the corresponding edges to upgrade to achieve such flow. 
	%If $\alpha$ is upper bound, then we can put that many copies of the edge to reduce it to this.
%\end{proof}

%Note that the above reduction also works for directed graphs. 
%Continuous upgrading of st-Minimum Cuts done in previous paper see intro


\iffalse ---------------------------------------------
\subsection{Bulk MinCut Upgrade is DkS Hard under bulk modification even with unitary upgrade costs}

\begin{lemma}
	MaxMC with unit upgrading cost $c$ is DkS hard. In particular, an $(\alpha, \beta)$-approximation to MaxMC yields a $8\alpha\beta^2$-approximation to DkS. 
\end{lemma}

\begin{proof}
	Given an instance of DkS let $G'$ be a graph where $V(G')=S\cup T\cup \{s, t\}$, and $S, T$ are simply copies of $V(G)$. Then, for every $u\in S, v\in T$, $uv\in E(G')$ if and only if $uv\in E(G)$. Also connect $s$ to ever vertex in $S$ and $t$ to every vertex in $T$. Every edge incident to $s, t$ has original capacity of 0, upgrade cost of 1 and an additional upgraded capacity of $\infty$ (or a very large number). Every edge between $S, T$ has original cost of $1$, upgrading cost of $1$ and additional capacity of $0$ (i.e., such edges cannot be upgraded). Note the current max-flow is $0$ and any solution would only want to upgrade edges incident to $s, t$. Let $b=2k$.
	
	Suppose we obtain a bicritera approximation solution for MaxMC on $G'$ where we upgrade $X'\subseteq E(G')$, resulting in a max-flow of $f^*/\alpha$ and $|X|=\beta 2k$. Let $Y$ be the set of vertices $v$ such that at least one of $sv, vt\in X$. Note that $f^*/(2\alpha)$ is a lower bound on the number of edges within $Y$ and $|Y|\le \beta 2k$. Then, using an averaging argument, there exists a $k$-subset within $Y$ with at least $f^*/(8\alpha\beta^2)$ edges. Since a solution to DkS easily corresponds to a solution of MaxMC for $G'$, $f^*$ is an upper bound on the number of edges in DkS. Then, our result follows.  
\end{proof}
	
This leads us to a new model where rather than require $\alpha(e)$ to be unitary for all edges, we allow an edge to be upgraded upto some maximum amount $u(e)$ but the cost per unit amount of upgrade is $c(e)$. We call such modifications where there is a cost per unit of modification `smooth'. 
------------------------------------------------------
\fi
	
	
\subsection{Discrete MinCut (or MaxFlow) Upgrading is strongly polytime}

\begin{problem} (MMF)
	Given a directed graph $G$, $s, t\in V$, functions $w,c,u:E\to \mathbb{N}$ and a budget $B$, find $x$ that maximizes $f_x$, the $st$-max-flow for $w+x$ edge capacities, while ensuring $c_x := c \cdot x \le B$ and $x \le u$. 
\end{problem}

Because of the maxflow-mincut theorem \cite{FF62}, MMF and MaxMC are equivalent.

\begin{lemma}
	MMF is strongly solvable in strongly polynomial time. 
\end{lemma}

\begin{proof}
   % This is a proof analogous to the proof of lemma \ref{MSPPoly}.
    
	Consider the following LP (MMFLP) for solving MMF:
	\begin{align*}
		\max \qquad & \sum_{v : (s,v)\in E} f_{sv} &\\
		\text{s. t.} \qquad & f_{e} \le w(e) + x_e & \forall e\in A(G)\\
		& x_e \le u(e) & \forall e \in E \\
		& \sum_{u : (u,v)\in E} f_{uv} - \sum_{w : (v,w)\in E} f_{vw} = 0 &\forall v \in V\setminus \{s,t\}\\
		& \sum_{e\in E} c(e)x_e \le B & \\
		& f_e,x_e \ge 0 & \forall e \in A(G) \\
	\end{align*}
	It follows from the work of Ahuja and Orlin \cite{AO95} (Theorem 3)  that one can obtain an optimal solution to the above LP in strongly polynomial time. Let $F_{opt}$ be the optimal value of the above LP. Consider $F_0=\lfloor F_{opt}\rfloor$ be a guess to the integral optimal value of MMF (which is clearly upperbounded by $F_0$). Note that given an optimal fractional solution to MMF, one can easily reduce/reverse the flows to obtain a integral solution, $(f_0, x_0)$, that gives $F_0$ as an objective value. 
	
	Then, consider the following LP, (MMFLP2), derived from the previous one by swapping the objective flow function with the budget constraint:
	
	\begin{align*}
		\min \qquad & \sum_{e\in E} c(e)x_e &\\
		\text{s. t.} \qquad & f_{e} \le w(e) + x_e & \forall e\in E\\
		& x(e) \le u(e) & \forall e \in E \\
		& \sum_{u : (u,v)\in E} f_{uv} - \sum_{w : (v,w)\in E} f_{vw} = 0  &\forall v \in V\setminus \{s,t\}\\
		& \sum_{v : (s,v)\in E} f_{sv} = F_0& \\
		& f_e,x_e \ge 0 & \forall e \in E 
	\end{align*}
	
	Note that the fractional solution $(f_0, x_0)$ is a feasible solution to MMFLP2. Thus, an optimal solution to MMFLP2 has a cost less than $B$, making it also feasible to MMFLP. We now show that there is an optimal solution to MMFLP that is integral. 
	
	%We will show that the matrix representing the constraints is TU. If we color all the constraints the same color, summing over the coefficients of a particular variable, the flows associated to an edge incident to $t$ has a value of $-1$ while all other variables is at $0$. This is a proper bicoloring and thus the matrix is TU. 
	
	
	
	%Furthermore, an integer solution to this LP corresponds to an $R$ such that the maximum flow between $s$ and $t$ is at least $f_0$, since the constraints make $f_e$ in the LP to be a legal flow, and $\sum_{v : (s,v)\in E} f_{sv} = f_0$.	One simply needs to find $f_0$ such that the solution to the LP spends within the budget $b$ while $f_0+1$ exceeds the budget. Since $f_0\le f_{\emptyset}+b$, we can binary-search through the possible values to find the optimal $f_0$. 
	
    We can view MMFLP2 as a min-cost flow problem. For every edge $e$, consider adding a parallel edge $e'$ to create graph $G'$. Edge $e$ has a capacity of original weight $w_e$ with a cost of $0$ while $e'$ has capacity $u(e)$ with cost $c(e)$. Then, solving MMFLP2 is equivalent to finding a flow of $F_0$ with minimum cost. Since min-cost flow is strongly polytime solvable \cite{WiBook} and produces an integral solution, we also have an integral solution to MMF. 
    %TODO cite strongly polytime result for flow

\end{proof}

\begin{remark}
The result still holds if there are no upper bounds, since removing a constraint in the LP doesn't change anything to the proof.
\end{remark}

\newpage





==> MinSPUpgrading.tex <==
\subsection{Upgrading $st$-Shortest Paths}


%Continuous $st$-shortest path upgrading done in previous paper see intro

\iffalse------------------------------------------

\subsection{Add hardness of bulk version and if possible a short reduction when alpha is unitary as in the MinCut case}

If we allow the bulk upgrade to be large, this problem is the same as finding the $k$ most vital edges for shortest path. This has been shown to be NP-complete in \cite{bar98} and constant hard to approximate in \cite{Khachiyan2008}. 
----------------------------------------------------
\fi

\subsection{Shortest Path Upgrading is strongly polytime solvable}

\begin{problem} (MSP)
	Given a directed graph $G$, $s, t\in V$, functions $w, c, u:E\to \mathbb{N}$ and a budget $B$, find $x$ that maximizes $l_x$, the length of the shortest path from $s$ to $t$ for edge lengths $w+x$, while ensuring total cost $c_x := \sum x(e) \cdot c(e) \le B$ and $\forall e \in E, x(e) \le u(e)$. 
\end{problem}
	
\begin{theorem}
	MSP is strongly polytime solvable. 
	\label{MSPPoly}
\end{theorem}

\begin{proof}
%	From Lemma \ref{ContMSPPoly}, we re-use (MSPLP) :
    Consider the following LP formulation (MSPLP) for this problem:
	\begin{align*}
		\max \qquad & d_t &\\
		\text{s. t.} \qquad & d_v \le d_u+w(e)+x_e  & \forall e=uv\in A(G)\\
		& x_e \le u(e) &\forall e\in A(G)\\
		& \sum_{e\in A(G)} c(e)x_e \le B &\\
		&d_s=0&\\
	\end{align*}
	
	From works by Fulkerson and Harding \cite{FH77}, one can obtain an optimal and integral solution to Min Shortest Path upgrading problem in strongly polynomial time and thus an optimal solution to MSPLP. Let $l_{opt}$ be the optimal value to the above LP. Let $l_0=\lfloor l_{opt} \rfloor$ be a guess to the integral optimal value of MSP. Given an optimal solution to MSPLP, one can lower the value of some $x(e)$s to obtain a feasible solution that provides an objective value of $l_0$. 
	
	Then, consider the following LP (MSPLP2) derived by swapping the objective function and the budget constraint :
	
	\begin{align*}
		\min \qquad & \sum_{e\in A(G)} c(e)x_e &\\
		\text{s. t.} \qquad & d_u+w(e)+x_e \ge d_v & \forall e=uv\in A(G)\\
		& x_e \le u(e) &\forall e\in A(G)\\
		&d_s=0, d_t \ge l_0 &\\
	\end{align*}
	
	Note that the feasible solution to MSPLP with objective value $l_0$ is also a feasible solution to MSPLP2. Thus, an optimal solution to MSPLP2 has an objective of at most $B$. We now show that there exists an optimal solution that is also integral. 
	
	%One way is to show that the matrix representing the constraints is TU. If we color all variables the same color, this provides a proper bicoloring of the constraints. Thus, we know the constraint matrix is TU and the above LP is poly-time solvable and integral. 
	
	%Furthermore, an integer solution to this LP corresponds to an $x$ such that the distance from $s$ to $t$ is at least $l_0$. Indeed, since $d_s = 0$ and $d_j - d_i \le w(ij)+x_{ij}$, by adding these constraints along the shortest path from $s$ to $t$, we get $d_t \le \sum_{e \in path} w(e)+x_{e}$. But $d_t \ge l_0$, so we do get that the shortest path is longer then $l_0$.
	
	%One simply needs to find $l_0$ such that the solution to the LP spends within the budget $b$ while $l_0+1$ exceeds the budget. Since $l_0\le l_{\emptyset}+b$, we can binary-search through the possible values to find the optimal $l_0$. 
	
	One can replace the last constraint in MSPLP2 with $d_t-d_s\ge l_0$ and take the dual to obtain the following:
	
		\begin{align*}
		\max \qquad & f_{ts}l_0-\sum_{e\in A(G)} w_ef_e &\\
		\text{s. t.} \qquad & \sum_{u\in N^-(v)}f_{uv}=\sum_{w\in N^+(v)}f_{vw} & \forall v\in V(G)\backslash \{s, t\}\\
		& \sum_{u\in N(s)}f_{su}=f_{ts} &\\
		& \sum_{w\in N(s)}f_{wt}=f_{ts} &\\
        & f_{uv}\le r_{uv} & \forall uv\in A(G)\\
    	\end{align*}
    	
    If we add an arc from $t$ to $s$ with cost $-l_0$ and associate a cost of $w_e$ to every arc $e$, the above is equivalent to a min-cost circulation problem. We know this is strongly polytime solvable \cite{WiBook} and has an integral solution with integral objective values if all coefficients are integral. Given the integral solution, one can easily obtain an integral dual solution and thus revert back to an integral solution to MSPLP2 and thus MSP. This certifies $l_0$ is the optimal value and provides us an integral optimal solution. 
\end{proof}
%TODO ask Da Qi
	
\newpage

==> cover.tex <==
\noindent To Editors of ACM Transactions on Algorithms, 

\null    

One of the main contributions in this paper is to correct an error in \cite{FS96}: Increasing the Weight of Minimum Spanning Trees by Frederickson and Solis-Oba. In \cite{FS96}, they provided an optimal solution via a polynomial-time algorithm to a particular perturbation problem. Although their algorithm is correct, their analysis is flawed. We point out this mistake and provide a correct proof.

Since their same idea and incorrect proof were also used in a later paper to solve a more general problem \city{FS98}, we believe it is important for the community to be aware of this issue and its resolution. Our paper also include approximation algorithms for other related perturbation problems. 

\null
\null


\noindent Sincerely, 

\null

\noindent
Coauthors of this manuscript

==> overflow.tex <==
%\input{MinCutUpgrading}
%\input{MinSPUpgrading}

\section{Observations about MST Downgrading}
\begin{definition}
If $(G,w,c,B)$ is an instance of MMST, then if $x$ is a downgrading scheme such that :
\begin{itemize}
    \item $f_x = max\{f_{x'} | c_{x'} \le B\}$
    \item $c_x = min\{c_{x'} | f_{x'} = f_x\}$
\end{itemize}
then we call $x$ an \textit{optimal downgrading scheme}.
\end{definition}

\begin{remark}
    If $(G,w,c,B)$ is an instance of MMST, and we have an optimal downgrading scheme $x$, then the sets of MSTs in $(G,w)$ and $(G,w+x)$ can have an empty intersection. See counterexample in Figure \ref{CounterEx0}.
    
\begin{figure}[h]
\begin{center}
\begin{tikzpicture}[thick]
	\node[shape=circle,draw=black] (A) at (-2,0) {$A$};
	\node[shape=circle,draw=black] (B) at (2,0) {$B$};
	\node[shape=circle,draw=black] (C) at (0,2) {$C$};
	
	\draw (A) to (B);
    \draw (B) to (C);
    \draw (C) to (A);
	\node at (0,-0.3) {$w = 2, c = 20$};
	\node at (-2,1) {$w = 1, c = 1$};
	\node at (2,1) {$w = 1, c = 1$};
\end{tikzpicture}
\end{center}
\caption{The MST at the start is \{AC,CB\}. With budget 4, the MSTs at the end are \{AB,AC\}  and \{AB,BC\}.}
\label{CounterEx0}
\end{figure}

\end{remark}


\iffalse
\begin{proof}

NOT TRUE
Let $x$ be an optimal downgrading scheme. Let us call $M_1$ the set of MSTs in $(G,w)$ and $M_2$ the set of MSTs in $(G,w+x)$.
We aim to prove by contradiction that $M_1 \cap M_2 \ne \emptyset$. Let us suppose that $M_1 \cap M_2 = \emptyset$.

We now create a series of downgrading schemes, $x_0,...,x_k = x$, where (seen as multisets) $x_{i} \subset x_{i+1}$ and $\#x_{i} = i$. 

For $e$ an edge in $G$, let $w_{x_i}(e)$ be the weight of $e$ after the downgrading scheme $x_i$, that is $w_{x_i}(e) = w(e) + x_i(e)$.
If $S$ is a set of sets of edges (such as $M_1$) then $w_{x_i}(S) = min\{w_{x_i}(T) | T \in S \}$.
Then, we know that $w_{x_0}(M_1) < w_{x_0}(M_2)$ and $w_{x_k}(M_1) > w_{x_0}(M_2)$. We also know that $w_{x_{i+1}}(M_j) - w_{x_{i}}(M_j) \le 1$, for $j \in \{1,2\}$. Thus, for some index $i$, $w_{x_i}(M_1) = w_{x_i}(M_2)$ and $w_{x_{i+1}}(M_1) > w_{x_{i+1}}(M_2)$. Let $f$ be the edge downgraded between $x_{i}$ and $x_{i+1}$.

We now introduce $x'(e) := \left\{
    \begin{array}{ll}
        x(e)-1 & \mbox{if } e = f \\
        x(e) & \mbox{otherwise.}
    \end{array}
\right.$

We notice first of all that clearly $c_{x'} < c_{x}$.
We now prove that $x'$ is a downgrading scheme such that $f_{x'} = f_x$ thus giving us a contradiction, since $x$ is not optimal.

Let $T$ be an MST for $x'$. Then $w_x'(T) \le w_x'(M_2)$, and so $w_x(T) \le w_x'(T) + 1 \le w_x'(M_2) + 1 \le w_x(M_2)+1$, and furthermore $w_x(T) \ge w_x(M_2)$. Thus all the inequalities are equalities, and $T \in M_2$ (by definition of $M_2$).
Thus all MSTs for $x'$ are in $M_2$.

Furthermore, we know that $w_{x_i}(M_2) = w_{x_{i+1}}(M_2)$, and so $w_{x'}(M_2) = w_{x}(M_2)$. %Why is this true ? Actually, is it true ? I don't think it is true... Because you could have an edge that downgrades a non minimal tree in x_i, but that is actually minimal in x...
\end{proof}
\fi


\begin{lemma}
Let $x$ be an optimal downgrading scheme, $T$ be an MST for $(G,w_x)$, and $e_0$ an edge such that $x(e_0) > 0$ and $e_0 \notin T$. Let $C$ be the cycle created by $T+e_0$. Then we have :
$$w_x(e_0) = \max_{e\in C-e_0}\{w_x(e)\}$$
\end{lemma}

\begin{proof}
First of all, since $T$ is an MST, $\forall e \in C, w_x(e_0) \ge w_x(e)$. And so, 
$$w_x(e_0) \ge \max_{e\in C-e_0}\{w_x(e)\}$$

Now, let $x'(e) := \left\{
    \begin{array}{ll}
        x(e)-1 & \mbox{if } e = e_0. \\
        x(e) & \mbox{otherwise.}
    \end{array}
\right.$ \\
Since $x$ optimal downgrading scheme, all MSTs in $(G,w_{x'})$ contain $e_0$, otherwise $x'$ would be a less costly downgrading scheme for the same MST weight. \\
Let $T'$ be an MST in $(G,w_{x'})$. Since $e_0 \in T'$, $T'-e_0$ has two components, separated by a cut $\delta$, which contains $e_0$.  \\
Let $e \in \delta \setminus \{e_0\}$. Then $T'-e_0 + e$ is a tree which does not contain $e_0$, and is thus not an MST. Thus $w_{x'}(T'-e_0+e) > w_{x'}(T')$, and so $w_{x'}(e_0) < w_{x'}(e)$ thus $w_{x}(e_0) \le w_{x}(e)$ and that is the case for all $e \in \delta \setminus \{e_0\}$. \\
$C$ contains $e_0$, so at least one edge of $\delta$. Since $C$ is a cycle and $\delta$ is a cut, $|C \cap \delta| \ge 2$. Let $e \in C \cap \delta \setminus \{e_0\}$. We have $w_{x}(e_0) \le w_{x}(e)$ and $w_{x}(e_0) \ge w_{x}(e)$, and so $w_{x}(e_0) = w_{x}(e)$. Finally we have:
$$w_x(e_0) = \max_{e\in C-e_0}\{w_x(e)\}$$
\end{proof}

\begin{corollary}
If we have a final MST and the upgraded value of the edges in that tree, then we know everything we need to downgrade, and the cost.
\end{corollary}

\newpage



\section{Downgrading MSTs when all initial edge weights are identical}

*** RESTATE as 1/2 and additive one less

Here we discuss a simpler version of problem.  Assume that every edge $e \in E(G)$ has the same original weight $l_0$ and let $x_e$ denote the amount by which the length can be increased with a per unit cost $c(e)$.  Given a target value $t > (n-1)l_0$,  the problem of increasing the length of all the spanning trees to at least $t$ can be written as 

\begin{equation*}
\begin{split}
\mbox{minimize} \quad & \sum c(e) x_e\\
\mbox{such that} \quad & \sum_{e \in T} x_e \ge t - (n-1)l_0 \quad \forall \text{ Spanning Trees } T\\
& x_e \ge 0 \quad \forall e \in E(G)\\
\end{split}
\end{equation*}

Its dual corresponds to the problem of packing spanning trees.

\begin{equation*}
\begin{split}
\mbox{maximize} \quad & (t - (n-1)l_0)\sum y_T\\
\mbox{such that} \quad & \sum_{T \ni e} y_T \le c(e) \quad \forall e \in E(G)\\
& y_T \ge 0 \quad \forall \text{ Spanning Trees } T\\
\end{split}
\end{equation*}

Let $y^*$ denote an optimal solution of the dual problem.  Tutte and Nash Williams showed that 

$$\sum y^*_T = \min_{\mathcal{P}}\frac{c(\mathcal{P})}{\vert \mathcal{P} \vert-1},$$

\noindent where $\mathcal{P}$ is a partition of the vertex set $V(G)$,  $\vert \mathcal{P} \vert$ denote the number of its parts,  and $c(\mathcal{P})$ denote its cost.  Let $\mathcal{P}^*$ denote the partition that achieves the minimum and $\lambda(G)$ denote the value of the global minimum cut of $G$.  It is known that

$$(t - (n-1)l_0) \sum y^*_T = \frac{(t - (n-1)l_0) c(\mathcal{P}^*)}{\vert \mathcal{P}^* \vert-1} \ge \frac{(t - (n-1)l_0) \vert \mathcal{P}^* \vert }{2(\vert \mathcal{P}^* \vert-1)}\lambda(G) \ge \frac{(t - (n-1)l_0) n }{2(n-1)}\lambda(G).$$

Therefore,  the cost of increasing the length of any edge in any global minimum cut by $\lfloor \frac{(t - (n-1)l_0) n }{2(n-1)}\rfloor$ is bounded by $b$ and  the length of any spanning tree increases by at least

$$\lfloor \frac{(t - (n-1)l_0) n }{2(n-1)} \rfloor \ge \frac{(t - (n-1)l_0) n }{2(n-1)} - \frac{1}{2}$$

--------Old

\begin{lemma}
Suppose all edges start with weight $w_0$, and there is an optimal downgrading scheme that downgrades every edge at least once. Then we get a $\frac{opt}{2}-1$-approximation, where $opt$ s the optimal increase in the weight of the MST.
\end{lemma}

\begin{proof}
We swap the target increase, which we call $t$, and the budget constraint, in order to get this LP :
\begin{equation*}
\begin{split}
\mbox{minimize} \quad & \sum c(e) x_e\\
\mbox{such that} \quad & \sum_{e \in T} x_e \ge t - (n-1)w_0 \quad \forall \text{ Spanning Trees } T\\
& x_e \ge 0 \\
\end{split}
\end{equation*}
This has a dual LP :
\begin{equation*}
\begin{split}
\mbox{maximize} \quad & (t - (n-1)w_0)\sum y_T\\
\mbox{such that} \quad & \sum_{T \ni e} y_T \le c(e) \quad \forall e \in E(G)\\
& y_T \ge 0 \\
\end{split}
\end{equation*}
Now, suppose that $\forall e, x^*_e > 0$ is an optimal solution to the first LP, with $t^*$ such that $\sum c(e) x^*_e = B$. Then we have

\begin{align*}
	\sum_T y^*_T & = \sum_T y^*_T \sum_{e \in T} \frac{1}{n-1} = \frac{1}{n-1} \sum_e  \sum_{T \ni e} y^*_T \\
	& =\frac{1}{n-1} \sum_e  c(e) \quad \text{By complementary slackness} \\
	& = \frac{1}{2(n-1)} \sum_v deg(v,\text{cost } c(e)) \\
	& > \frac{1}{2n} \sum_v deg(v,\text{cost } c(e)) \\
	& \ge \frac{1}{2} \sum_v min\_cut(\text{cost } c(e))
\end{align*}
And so, the increase we get if we lift this minimum cut until we don't have enough budget is :
\begin{align*}
    \text{increase} & = \lfloor \frac{B}{min\_cut} \rfloor > \frac{B}{min\_cut} -1 \\
    & > \frac{B(t - (n-1)w_0)}{2(t - (n-1)w_0)\sum_T y^*_T } -1 \\
    & = (t - (n-1)w_0)\frac{B}{2B} -1 \\
    & = \frac{1}{2}(t - (n-1)w_0)-1
\end{align*}
We thus get a similar approximation to the one in Lemma 5.
\end{proof}

*** NOTE: Directed version of above is poly-time solvable with arborescence packing.


==> unit-UB-MST.tex <==
\section{Fortification of MSTs with unit upper bounds}

ADD section here on reducing the unit UB case to k-cut and vice-versa for the target version and correspondingly with max-components for the budget version.
